Logic Programming and Logarithmic Space

We present an algebraic view on logic programming, related to proof theory and more specifically linear logic and geometry of interaction. Within this construction, a characterization of logspace (deterministic and non-deterministic) computation is given via a synctactic restriction, using an encoding of words that derives from proof theory. We show that the acceptance of a word by an observation (the counterpart of a program in the encoding) can be decided within logarithmic space, by reducing this problem to the acyclicity of a graph. We show moreover that observations are as expressive as two-ways multi-heads finite automata, a kind of pointer machines that is a standard model of logarithmic space computation.

==> simple_example.tex <==
We give in \autoref{fig-state-diagram} the (labeled) state diagram of a deterministic automata\footnote{That is, with one head.} that ends on input $W \in \{0, 1\}^*$ if and only if $\exists n \in \natural$ such that $W = \start 0^n$.
Elsewhere, it loops by repeating the computation for ever.
We assume, for the sake of simplicity, that the head starts on the first bit next to $\start$, that the input is cyclic and that $\start$ occurs only once in $W$.
\CLEM{À clarifier dans la façon dont on définit un mot, et dont on le représente.}

\begin{figure}
\begin{minipage}[b]{0.45\textwidth}
\centering%
\begin{tikzpicture}[auto]%[shorten >=1pt,node distance=2cm,on grid,auto] 
   \node[state] (i)   {$\state{i}$}; 
   \node[state, accepting] (y) [below left=of i] {$\state{y}$}; 
   \node[state] (n) [below right=of i] {$\state{n}$}; 
    \path[->] 
    (i)		edge	[loop above]	node	{$0$}	node[pos=0.9,right]{\small{$t_1$}}		()
          	edge  	[bend right] 	node	{$1$} 	node[pos=0.9,left]{\small{$t_2$}}		(n)
           	edge  					node	{$\start$} node[pos=0.9,right]{\small{$t_6$}}	(y)
    (n)		edge	[loop below]	node	{$0$} 		node[pos=0.9,left]{\small{$t_3$}}	()
    		edge	[loop right]	node	{$1$} 		node[pos=0.9,below]{\small{$t_4$}}	()
           	edge  	[bend right]	node [swap]	{$\start$} node[pos=0.9,right]{\small{$t_5$}} (i);
\end{tikzpicture}%
\caption{A labeled state diagram for an automata that accepts $\start 0^n$}\label{fig-state-diagram}
\end{minipage}
\hspace{0.1\textwidth}
\begin{minipage}[b]{0.45\textwidth}
\centering%
\begin{align*}%
\wordterm{0}{\R}{\state{i}}{v}{z} & \rflow \wordterm{0}{\L}{\state{i}}{v}{z'} \tag{\small{$t_1$}} \label{set1}\\
\wordterm{1}{\R}{\state{i}}{v}{z} & \rflow \wordterm{1}{\L}{\state{n}}{v}{z'} \tag{\small{$t_2$}} \label{set2}\\
\wordterm{0}{\R}{\state{n}}{v}{z} & \rflow \wordterm{0}{\L}{\state{n}}{v}{z'} \tag{\small{$t_3$}} \label{set3}\\
\wordterm{1}{\R}{\state{n}}{v}{z} & \rflow \wordterm{1}{\L}{\state{n}}{v}{z'} \tag{\small{$t_4$}} \label{set4}\\
\wordterm{\start}{\R}{\state{n}}{v}{z} & \rflow \wordterm{\start}{\L}{\state{i}}{v}{z'} \tag{\small{$t_5$}} \label{set5}\\
\wordterm{\start}{\R}{\state{i}}{v}{z} & \rflow \wordterm{\start}{\L}{\state{y}}{v}{z'} \tag{\small{$t_6$}} \label{set6}
\end{align*}%
\caption{The corresponding encoding as flows}\label{fig-flow}
\end{minipage}
\end{figure}

We will now encode it as an observation.
Remember from \autoref{word-rep} that the string $W = \start \TT{c_1} \hdots \TT{c_n}$ over $\{\start, 0, 1\}$ with $\start$ occurring only once is represented, once the constant representing the positions $\extlist{\TT p_0}{\TT p_n}$ has been fixed, as 
\[
\begin{array}{llrcl}
	W :=	& & \wordterm{\start}{\L}{x}{y}{\TT{p_0}} & \sflow &  \wordterm{c_1}{\R}{x}{y}{\TT{p_1}} \\
			&+& \wordterm{c_1}{\L}{x}{y}{\TT{p_1}} & \sflow & \wordterm{c_2}{\R}{x}{y}{\TT{p_2}} \\
			& & & \vdots  \\
			&+& \wordterm{c_n}{\L}{x}{y}{\TT{p_n}} & \sflow & \wordterm{\start}{\R}{x}{y}{\TT{p_0}}
	\end{array}
\]

We denote by $a \rflow b$ the flow $b \flow a$: in the case of a transition system as the one we are going to expose, it helps to read it as a functional relation (here, a function) encoding a classical transition function. 

The observation will simply be the sum of the flows \eqref{set1}--\eqref{set6} given in \autoref{fig-flow}.
The variable $v$ stands for \enquote{void}: it will be of no use in this case, where only one head is used.

The fact that no flow has for state $\state{y}$ on its left-hand reflect the fact that this state is terminal: once this state is reached, no transition can take place.
In fact, one could even replace \eqref{set6} with
\begin{align*}%
\wordterm{\start}{\R}{\state{i}}{v}{z} & \rflow 0 \tag{\small{$t'_6$}} \label{set6bis}
\end{align*}%
Here, a loop is in fact a \enquote{perform for ever the same computation}.
There is a reason for this design: as the observation is a sum, any transition that can be applied will be applied, i.e. if the left-member of a flow of our observation and a part of the input can be unified, the computation will start in a possibly \enquote{wrong} initialization.
That some of this incorrect runs accept for incorrect reason is no trouble, since only rejection is meaningful in our framework.
Hence, the state $\state{n}$ acts as a buffer, where the head scans the input looking for the $\start$, and when it found it, it start the computation in the correct position, and in the correct state (that is, $\state{i}$).
Several runs occur in parallel, but we know that if the letter $1$ is ever found, all paths end.
On the contrary, if the letter $1$ is found, at least one path performs the computation forever.

Hence, this observation is nilpotent if and only if when applied to a representation of $W$, $W$ contains only $\start$ and $0$'s.

\CLEM{Faire un petit exemple d’entrée et de jeu programme / entrée ?}
